Reach-Avoid Control Synthesis for a Quadrotor UAV with Formal Safety Guarantees

Reach-avoid specifications are one of the most common tasks in autonomous aerial vehicle (UAV) applications. Despite the intensive research and development associated with control of aerial vehicles, generating feasible trajectories though complex environments and tracking them with formal safety guarantees remain challenging. In this paper, we propose a control framework for a quadrotor UAV that enables accomplishing reach-avoid tasks with formal safety guarantees. In this proposed framework, we integrate geometric control theory for tracking and polynomial trajectory generation using Bezier curves, where tracking errors are accounted for in the trajectory synthesis process. To estimate the tracking errors, we revisit the stability analysis of the closed-loop quadrotor system, when geometric control is implemented. We show that the tracking error dynamics exhibit local exponential stability when geometric control is implemented with any positive control gains, and we derive tight uniform bounds of the tracking error. We also introduce sufficient conditions to be imposed on the desired trajectory utilizing the derived uniform bounds to ensure the well-definedness of the closed-loop system. For the trajectory synthesis, we present an efficient algorithm that enables constructing a safe tube by means of sampling-based planning and safe hyper-rectangular set computations. Then, we compute the trajectory, given as a piecewise continuous Bezier curve, through the safe tube, where a heuristic efficient approach that utilizes iterative linear programming is employed. We present extensive numerical simulations with a cluttered environment to illustrate the effectiveness of the proposed framework in reach-avoid planning scenarios.

==> OldStuff.tex <==
% \section{Linear Constraints on the desired trajectory}

% \textbf{Recall the definitions of $V_{1}$ and $V_{2}$ above. Assume the control gains are already determined. Let the parameters $0<\bar{\Psi}$, $\alpha_{\psi}<1$ and $\bar{V}_{1}>0$ be chosen.  Assume the initial conditions of the quadrotor model $(p(0),v(0),R(0),\omega(0))$ are given (it would be nice if these conditions are non-zero).
% Find a set of linear constraints on $p_{d}(0),~p'_{d}(0), p''_{d}(0), p_{d}^{(3)}(0)$ such that  
% \begin{align*}
% V_{1}(0)&\leq \bar{V}_{1},\\
% \Psi(R(0), R_d(0))&\leq \alpha_{\psi}\overline{\Psi}\\
% \|e_\omega(0)\|^2 &\leq   \frac{2k_{R}}{\lambda_{max}(J)}(1-\alpha_{\psi})\overline{\Psi}.
% \end{align*}
% }
% Note that satisfying the above constraints ensure ${V}_{2}(0)\leq k_{m}\bar{\Psi}$, where  $k_{m}$ is defined above. So $V_{2}(0)$ can be ensured to be sufficiently small by letting $\bar{\Psi}$ be sufficiently small. 


% \begin{lemma} (Linear constraints for position and velocity)

%     Define $$\underline{\alpha}_1^2 = \frac{\bar{V}_{1}}{2\lambda_{max}(M_{1,2})}, \overline{\alpha}_1^2 = \frac{\min\{V_1(0), \bar{V}_{1}\}}{\lambda_{min}(M_{1,1})},$$ 
%     then if $$|\Delta x(0)|, |\Delta y(0)|, |\Delta z(0)| \leq \frac{\underline{\alpha}_1}{\sqrt{3}}, |\Delta v_x(0)|, |\Delta v_y(0)|, |\Delta v_z(0)| \leq \frac{\underline{\alpha}_1}{\sqrt{3}},$$
%     we have $$|\Delta x(t)|, |\Delta y(t)|, |\Delta z(t)| \leq \overline{\alpha}_1, |\Delta v_x(t)|, |\Delta v_y(t)|, |\Delta v_z(t)| \leq \overline{\alpha}_1, \forall t > 0.$$
% \end{lemma}

% \begin{proof}
%     \begin{align*}
%         & |\Delta x(0)|, |\Delta y(0)|, |\Delta z(0)| \leq \frac{\underline{\alpha}_1}{\sqrt{3}}, |\Delta v_x(0)|, |\Delta v_y(0)|, |\Delta v_z(0)| \leq \frac{\underline{\alpha}_1}{\sqrt{3}}\\
%         \Longleftrightarrow
%         & \max\{|\Delta x(0)|, |\Delta y(0)|, |\Delta z(0)|\} \leq \frac{\underline{\alpha}_1}{\sqrt{3}}, \max\{|\Delta v_x(0)|, |\Delta v_y(0)|, |\Delta v_z(0)|\} \leq \frac{\underline{\alpha}_1}{\sqrt{3}}\\
%         \Longleftrightarrow
%         & \sqrt{3}\|e_p(0)\|_\infty \leq \underline{\alpha}_1, \sqrt{3}\|e_v(0)\|_\infty \leq \underline{\alpha}_1\\
%         \Longrightarrow
%         & \|e_p(0)\|_2 \leq \underline{\alpha}_1, \|e_v(0)\|_2 \leq \underline{\alpha}_1\\
%         \Longleftrightarrow
%         & \max\{\|e_p(0)\|_2, \|e_v(0)\|_2\} \leq \underline{\alpha}_1\\
%         \Longleftrightarrow
%         & \|z_1(0)\|_\infty^2 \leq \underline{\alpha}_1^2 = \frac{\bar{V}_{1}}{2\lambda_{max}(M_{1,2})}\\
%         \Longrightarrow
%         & \lambda_{max}(M_{1,2}) \|z_1(0)\|_2^2 \leq \bar{V}_{1}
%     \end{align*}
% The Lyapunov analysis above gives
% $$
% \lambda_{min}(M_{1,1}) \|z_1\|_2^2 \leq z_{1} \cdot M_{1,1} \cdot z_{1} \leq V_{1}\leq z_{1} \cdot M_{1,2} \cdot z_{1} \leq \lambda_{max}(M_{1,2}) \|z_1\|_2^2.
% $$
% then we have $\lambda_{min}(M_{1,1}) \|z_1(t)\|_2^2 \leq \bar{V}_{1}$, or $\|z_1(t)\|_2^2 \leq \overline{\alpha}_1$. Then,
%     \begin{align*}
%         & \|z_1\|_2^2 \leq \overline{\alpha}_1\\
%         \Longrightarrow
%          & \|z_1\|_\infty^2 \leq \overline{\alpha}_1\\
%         \Longleftrightarrow
%         & \max\{\|e_p\|_2, \|e_v\|_2\} \leq \overline{\alpha}_1\\
%         \Longleftrightarrow
%         & \|e_p\|_2 \leq \overline{\alpha}_1, \|e_v\|_2 \leq \overline{\alpha}_1\\
%         \Longrightarrow
%         & \|e_p\|_\infty \leq \overline{\alpha}_1, \|e_v\|_\infty \leq \overline{\alpha}_1\\
%         \Longleftrightarrow
%         & \max\{|\Delta x|, |\Delta y|, |\Delta z|\} \leq \overline{\alpha}_1, \max\{|\Delta v_x|, |\Delta v_y|, |\Delta v_z|\} \leq \overline{\alpha}_1\\
%         \Longleftrightarrow
%         & |\Delta x|, |\Delta y|, |\Delta z| \leq \overline{\alpha}_1, |\Delta v_x|, |\Delta v_y|, |\Delta v_z| \leq \overline{\alpha}_1
%     \end{align*}
% \end{proof}

% \begin{lemma}
%     Given $\Psi(R, R_d) \leq \alpha_{\psi}\overline{\Psi}$, assume yaw $\psi = 0$, we have the bounds for roll $\phi$ and pitch $\theta$ as follows:
%     $$- \arccos(\sqrt{4-2\alpha_{\psi}\overline{\Psi}}-1) \leq \phi - \phi_d, \theta - \theta_d \leq \arccos(\sqrt{4-2\alpha_{\psi}\overline{\Psi}}-1)$$
% \end{lemma}

% \begin{proof}
%     Assume $\psi = 0$, let $R_{ref} = R_d^{\intercal}R$, $\theta_{ref} = \theta - \theta_d$, $\phi - \phi_d$, the relative rotation matrix is 
%     $$R_{ref} = \begin{bmatrix}
%         \cos \theta_{ref} & \sin \phi_{ref} \sin \theta_{ref} & \cos \phi_{ref} \sin \theta_{ref}\\
%         0 & \cos \phi_{ref} & - \sin \phi_{ref} \\
%         -\sin \theta_{ref} & \sin \phi_{ref} \cos \theta_{ref} & \cos \phi_{ref} \cos \theta_{ref}
%         \end{bmatrix}.$$
%     Then $$\tr(R_{ref}) = \cos \phi_{ref} + \cos \theta_{ref} + \cos \phi_{ref} \cos \theta_{ref} = 1 + 2 \cos \gamma,$$ where $\gamma$ is the angle in angle-axis representation. Given $$\Psi(R, R_d) = 1 - \cos \gamma \leq \alpha_{\psi}\overline{\Psi},$$
%     we have $$\cos \gamma \geq 1 - \alpha_{\psi}\overline{\Psi}.$$
%     Then $$\cos \phi_{ref} + \cos \theta_{ref} + \cos \phi_{ref} \cos \theta_{ref} \geq 3 - 2(\alpha_{\psi}\overline{\Psi}).$$
%     Set $\zeta = \cos \phi_{ref} = \cos \theta_{ref}$ and solve $$2 \zeta + \zeta^2 \geq 3 - 2(\alpha_{\psi}\overline{\Psi}),$$
%     we have $$\sqrt{4-2\alpha_{\psi}\overline{\Psi}}-1) \leq \cos \phi_{ref}, \cos \theta_{ref} \leq 1,$$ or $$- \arccos(\sqrt{4-2\alpha_{\psi}\overline{\Psi}}-1) \leq \phi_{ref}, \theta_{ref} \leq \arccos(\sqrt{4-2\alpha_{\psi}\overline{\Psi}}-1)$$
% \end{proof}

% \begin{lemma}
%     Angular velocities $\dot{\phi}, \dot{\theta}$ can be expressed as functions of derivatives of flat outputs as follows:
%     $$\dot{\phi} = -\frac{m}{f}(\dddot{x}\sin \phi \sin \theta + \dddot{y} \cos \phi + \dddot{z} \sin \phi \cos \theta)$$
%     $$\dot{\theta} = \frac{m}{f}(\dddot{x} \cos \theta + \dddot{z} (- \sin \theta))$$
%     where the total force $f = m \sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}$
% \end{lemma}

% \begin{proof}

% From \cite{mellinger2011minimum} equation (7), we have angular velocities expressed as follows:
% $$\dot{\phi} = -\frac{m}{f}(\dot{a} - (\dot{a} \cdot z_b)z_b) \cdot y_b = -\frac{m}{f}\dot{a} \cdot y_b 
% = -\frac{m}{f}(\dddot{x}\sin \phi \sin \theta + \dddot{y} \cos \phi + \dddot{z} \sin \phi \cos \theta)$$
% $$\dot{\theta} = \frac{m}{f}(\dot{a} - (\dot{a} \cdot z_b)z_b) \cdot x_b = \frac{m}{f}\dot{a} \cdot x_b
% = \frac{m}{f}\dot{a} \cdot x_b = \frac{m}{f}(\dddot{x} \cos \theta + \dddot{z} (- \sin \theta))$$
% where the total force $f = m \sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}$.
% \end{proof}


% % Then, we plug in
% % $$\sin\phi = \frac{-\ddot{y}}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}}, \cos\phi = \frac{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}}$$
% % $$\sin\theta = \frac{\ddot{x}}{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}}, \cos\theta = \frac{\ddot{z} + g}{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}}$$
% % we have
% % \begin{equation}
% % \begin{split}
% %     \dot{\phi} = -\frac{1}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}} (& \frac{\ddot{x}}{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}} \frac{-\ddot{y}}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}} \dddot{x} \\ & + \frac{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}} \dddot{y} \\ & + \frac{-\ddot{y}}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}} \frac{\ddot{z}+g}{ \sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}} \dddot{z})
% % \end{split}
% % \end{equation}
% % \begin{equation}
% %     \dot{\theta} = \frac{1}{\sqrt{\ddot{x}^2 + \ddot{y}^2 + (\ddot{z}+g)^2}}(\frac{\ddot{z}+g}{ \sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}} \dddot{x} - \frac{\ddot{x}}{\sqrt{\ddot{x}^2 + (\ddot{z}+g)^2}} \dddot{z})
% % \end{equation}

% Assume $\dot{\phi}(0) = \dot{\theta}(0) = 0$, we have $\|\dot{\phi}_d(0)\|, \|\dot{\theta}_d(0)\| \leq \frac{\alpha_\omega}{\sqrt{3}}$.
% \begin{equation}
%     \begin{split}
%         \|\dot{\phi}_d\| & \leq \|\sin\theta_d\| \|\sin\phi_d\| \frac{m\|{\dddot{p}_d}_x\|}{\|f_{max}\|} + \|\cos\theta_d\| \frac{m\|{\dddot{p}_d}_y\|}{\|f_{max}\|} \\
%         & \quad + \|\cos\theta_d\| \|\sin\phi_d\| \frac{m\|{\dddot{p}_d}_z\|}{\|f_{max}\|} \leq \frac{\alpha_\omega}{\sqrt{3}} \\
%         \|\dot{\theta}_d\| & \leq \|\cos\theta_d\| \frac{m\|{\dddot{p}_d}_x\|}{\|f_{max}\|} + \|\sin\theta_d\| \frac{m\|{\dddot{p}_d}_z\|}{\|f_{max}\|} \leq \frac{\alpha_\omega}{\sqrt{3}}
%     \end{split}
% \end{equation}
% Given $\|\sin\phi_d(0)\| \leq \frac{\alpha_\omega}{\sqrt{3}}$, $\|\sin\theta_d(0)\| \leq \frac{\alpha_\omega}{\sqrt{3}}$, $\|\cos\theta_d(0)\| \leq 1$, we need
% \begin{equation}
%     \begin{split}
%         \|\dot{\phi}_d(0)\| & \leq (\frac{\alpha_\omega}{\sqrt{3}})^2 \frac{m\|{\dddot{p}_d}_x(0)\|}{\|f_{max}\|} +  \frac{m\|{\dddot{p}_d}_y(0)\|}{\|f_{max}\|} + \frac{\alpha_\omega}{\sqrt{3}} \frac{m\|{\dddot{p}_d}_z(0)\|}{\|f_{max}\|} \leq \frac{\alpha_\omega}{\sqrt{3}} \\
%         \|\dot{\theta}_d(0)\| & \leq \frac{m\|{\dddot{p}_d}_x(0)\|}{\|f_{max}\|} + \frac{\alpha_\omega}{\sqrt{3}} \frac{m\|{\dddot{p}_d}_z(0)\|}{\|f_{max}\|} \leq \frac{\alpha_\omega}{\sqrt{3}}
%     \end{split}
% \end{equation}
% Put the same weights on each term, we have
% \begin{equation}
% \begin{split}
%     \frac{m\|{\dddot{p}_d}_x(0)\|}{\|f_{max}\|} & \leq \gamma_x = \frac{1}{\sqrt{3} \alpha_\omega},\\
%     \frac{m\|{\dddot{p}_d}_y(0)\|}{\|f_{max}\|} & \leq \gamma_y = \frac{\alpha_\omega }{3\sqrt{3}},\\
%     \frac{m\|{\dddot{p}_d}_z(0)\|}{\|f_{max}\|} & \leq \gamma_z = \frac{1}{3}
% \end{split}
% \end{equation}
% So, 
% \begin{equation}
% \begin{split}
%      \|{\dddot{p}_d}_x(0)\| & \leq \min\{\frac{\|f_{max}\|}{\sqrt{3} m \alpha_\omega}, \frac{\alpha_\omega  \|f_{max}\|}{2 \sqrt{3} m}\}, \\
%      \|{\dddot{p}_d}_y(0)\| & \leq \frac{\alpha_\omega \|f_{max}\|}{3\sqrt{3} m}, \\
%      \|{\dddot{p}_d}_z(0)\| & \leq  \frac{\|f_{max}\|}{3 m}
% \end{split}
% \end{equation}





% \begin{lemma}
%     Let ($\boldsymbol{a}_{\Psi}$, $\theta_{\Psi}$) be the angle-axis representation of the rotation matrix $R_d^T R$. Then given $\theta_{\Psi} \in [0, \frac{\pi}{2}]$, we have 
%     $1 > e_3^{\intercal} R_d^{\intercal} Re_3 > 1 - \Psi > 0$. And $\frac{1}{e_3^T R_d^T R e_3}$ is well-defined.
% \end{lemma}

% \begin{proof}
%     Consider axis-angle representation of attitude use an axis $\boldsymbol{a}_{\Psi} = (a_1, a_2, a_3) \in \Re^3$ and an angle $\theta_{\Psi} \in [0, \frac{\pi}{2}]$, where $\|\boldsymbol{a}_{\Psi}\| = 1$. Then the relationship between the rotation matrix $R_d^T R$ and axis-angle representation ($\boldsymbol{a}_{\Psi}$, $\theta_{\Psi}$) is:
% \begin{equation}
%     \diag(R_d^TR) = \begin{bmatrix}
%         \cos \theta_{\Psi} + a_1^2(1-\cos \theta_{\Psi})\\
%         \cos\theta_{\Psi} + a_2^2 (1-\cos\theta_{\Psi})\\
%         \cos\theta_{\Psi} + a_3^2 (1-\cos\theta_{\Psi})
%     \end{bmatrix}
% \end{equation}
% $\Psi$ as a function of $\theta_{\Psi}$ is:
% \begin{equation}
%     \begin{split}
%         \Psi & = \frac{1}{2}tr[I - R_d^TR]\\
%         & = \frac{1}{2}[(1 - (\cos \theta_{\Psi} + a_1^2(1-\cos \theta_{\Psi})))\\
%         & \quad + (1 - (\cos \theta_{\Psi} + a_2^2(1-\cos \theta_{\Psi})))\\
%         & \quad + (1 - (\cos \theta_{\Psi} + a_3^2(1-\cos \theta_{\Psi})))]\\
%         & = 1-\cos\theta_{\Psi}
%     \end{split}
% \end{equation}
% Hence we have $e_3^T R_d^T R e_3$ and $1-\Psi$ as functions of ($\boldsymbol{a}_{\Psi}$, $\theta_{\Psi}$) as follows:
% \begin{equation}
%     \begin{split}
%         e_3^T R_d^T R e_3 & = (R^T R_d e_3) \cdot e_3\\
%         & = (R_d^T R e_3) \cdot e_3\\
%         & = \cos\theta_{\Psi} + a_3^2 (1-\cos\theta_{\Psi})
%     \end{split}
% \end{equation}
% \begin{equation}
%     1 - \Psi = \cos\theta_{\Psi}
% \end{equation}
% Given $\theta_{\Psi} \in [0, \frac{\pi}{2}]$, we have
% \begin{equation}
%     1 > e_3^T R_d^T R e_3 > 1 - \Psi > 0
% \end{equation}
% And hence $\frac{1}{e_3^T R_d^T R e_3}$ is well-defined.
% \end{proof}


% \begin{proof}[Proof of Lemma \ref{lem:PropertiesHat}]
%     From the definition of the hat map, we have
%     \begin{equation}
%         \hat{x}y = \begin{pmatrix} 
%             0 & -x_3& x_2\\
%             x_3 & 0 & -x_1\\
%             -x_2 & x_1 & 0
%             \end{pmatrix}
%             \begin{pmatrix}
%                 y_1\\y_2\\y_3
%             \end{pmatrix}\\
%             = \begin{pmatrix}
%                 x_2 y_3 - x_3 y_2\\
%                 x_3 y_1 - x_1 y_3\\
%                 x_2 y_1 - x_1 y_2
%             \end{pmatrix}
%             = x \times y = - y \times x = - \hat{y} x
%     \end{equation}
%     So \eqref{hat1} holds. 
    
%     For \eqref{hat2}, $\tr(A\hat{x}) = \frac{1}{2}(\tr(A \hat{x}) + \tr(\hat{x}A)) = \frac{1}{2}(\tr(A \hat{x}) + (- \tr(A^{\intercal}\hat{x}))) = \frac{1}{2} \tr((A - A^{\intercal}) \hat{x})$, $(A - A^{\intercal})$ is skew-symmetric. Let $(A - A^{\intercal})^\vee = [a_1, a_2, a_3]^{\intercal}$, then
% \begin{equation}
% \begin{split}
% \frac{1}{2}\tr((A - A^{\intercal}) \hat{x}) & = \frac{1}{2}\tr(\begin{pmatrix}
%                                 0 & -a_3 & a_2\\
%                                 a_3 & 0 & -a_1\\
%                                 -a_2 & a_1 & 0
%                              \end{pmatrix} \cdot
%                              \begin{pmatrix}
%                                 0 & -x_3 & x_2\\
%                                 x_3 & 0 & -x_1\\
%                                 -x_2 & x_1 & 0
%                              \end{pmatrix}) \\
%                         & = \frac{1}{2}\tr(\begin{pmatrix}
%               -a_3 x_3 - a_2 x_2 & .. & ..\\
%               .. & -a_3 x_3 - a_1 x_1 & ..\\
%               .. & .. & -a_2 x_2 - a_1 x_1
%                              \end{pmatrix}) \\
%                     & = - (a_1 x_1 + a_2 x_2 + a_3 x_3)\\
%                     & = - (A - A^{\intercal})^\vee \cdot x\\
%                     & = - x^{\intercal}(A - A^{\intercal})^\vee
% \end{split}
% \end{equation}

% To prove \eqref{hat3}, we take
% $$x = (x_1, x_2, x_3)^\intercal$$
% $$A = \begin{pmatrix}
%             a_{11} & a_{12} & a_{13} \\
%             a_{21} & a_{22} & a_{23} \\
%             a_{31} & a_{32} & a_{33}
%         \end{pmatrix}$$
% Then,
% \begin{equation}
%     \begin{split}
%         (\hat{x}A + A^{\intercal} \hat{x})^\vee & =
%         (\begin{pmatrix} 
%             0 & -x_3& x_2\\
%             x_3 & 0 & -x_1\\
%             -x_2 & x_1 & 0
%         \end{pmatrix}
%         \begin{pmatrix}
%             a_{11} & a_{12} & a_{13} \\
%             a_{21} & a_{22} & a_{23} \\
%             a_{31} & a_{32} & a_{33}
%         \end{pmatrix} +
%         \begin{pmatrix}
%             a_{11} & a_{21} & a_{31} \\
%             a_{12} & a_{22} & a_{32} \\
%             a_{13} & a_{23} & a_{33}
%         \end{pmatrix}
%         \begin{pmatrix} 
%             0 & -x_3& x_2\\
%             x_3 & 0 & -x_1\\
%             -x_2 & x_1 & 0
%         \end{pmatrix})^\vee\\
%         & = (\begin{pmatrix}
%             .. & x_1 a_{31} + x_2 a_{32} - x_3 (a_{22} + a_{11}) & -x_1 a_{21} + x_2 (a_{11} + a_{33}) - x_3 a_{23}\\
%             .. & .. & -x_1 (a_{22} + a_{33}) + x_2 a_{12} + x_3 a_{13}\\
%             .. & .. & ..
%         \end{pmatrix})^\vee\\
%         & = \begin{pmatrix}
%             x_1 (a_{22} + a_{33}) - x_2 a_{12} - x_3 a_{13}\\
%             -x_1 a_{21} + x_2 (a_{11} + a_{33}) - x_3 a_{23}\\
%             -x_1 a_{31} - x_2 a_{32} + x_3 (a_{22} + a_{11})
%         \end{pmatrix}\\
%         & = \begin{pmatrix}
%             a_{22} + a_{33} & - a_{12} & - a_{13}\\
%             - a_{21} & a_{11} + a_{33} & - a_{23}\\
%             - a_{31} & - a_{32} & a_{11} + a_{22}
%         \end{pmatrix}
%         \begin{pmatrix}
%             x_1\\x_2\\x_3
%         \end{pmatrix}\\
%         & = (\tr(A)I - A)x
%     \end{split}
% \end{equation}

% For \eqref{hat4}, we have
% \begin{equation}
% \begin{split}
% & \widehat{R\omega} = R \hat{\omega} R^{\intercal} \\
% \Longleftrightarrow & \widehat{R\omega} = R^{-T} \hat{\omega} R^{-1} \\
% \Longleftrightarrow & R^{\intercal} \widehat{R \omega} R = \hat{\omega} \\
% \Longleftrightarrow & y^{\intercal} R^{\intercal} \widehat{R \omega} Rx = y^{\intercal} \hat{\omega} x \hspace{1cm} \forall x, y \in R^3\\
% \Longleftrightarrow & y^{\intercal} R^{\intercal} (R \omega \times R x) = y^{\intercal} (\omega \times x) \hspace{1cm} \forall x, y \in R^3\\
% \Longleftrightarrow & (R y) \cdot (R \omega \times R x) = y \cdot (\omega \times x) \hspace{1cm} \forall x, y \in R^3 \\
% \Longleftrightarrow & \det(Ry, R\omega, Rx) = \det(y, \omega, x) \hspace{1cm} \forall x, y \in R^3 \\
% \Longleftrightarrow & \det(R)\det(y, \omega, x) = \det(y, \omega, x) \hspace{1cm} \forall x, y \in R^3 \\
% \Longleftrightarrow & \det(R) = 1 \\
% \end{split}
% \end{equation}
% Since $\det(R) = 1$ is always true for all $x, y \in R^3$ and $R \in \SO$, then \eqref{hat4} holds.
% \end{proof}







